DISCO---An HPSG-based NLP System and its Application for Appointment Scheduling (Project Note)

The natural language system DISCO is described. It combines o a powerful and flexible grammar development system; o linguistic competence for German including morphology, syntax and semantics; o new methods for linguistic performance modelling on the basis of high-level competence grammars; o new methods for modelling multi-agent dialogue competence; o an interesting sample application for appointment scheduling and calendar management.

==> 9406035.2 <==
\newfont{\hvdemi}{cmssdc10 scaled 650}
\newfont{\hvitalic}{cmssi10 scaled 660}
\newfont{\tinytt}{cmtt8 scaled 220}
\newfont{\smallsc}{cmcsc8 scaled 750}
\newfont{\smallsf}{cmss8 scaled 730}

\setlength{\unitlength}{0.5mm}

\begin{picture}(155,212.5)
  \thicklines
  \put(35,197.5){\line(1,0){110}}
  \put(35,197.5){\line(0,1){10}}
  \put(145,197.5){\line(0,1){10}}
  \put(35,197.5){\makebox(110,10){\hvdemi APPOINTMENT PLANNER }}
  \put(50,196.5){\vector(0,-1){13}}
  \put(130,183.5){\vector(0,1){13}}
  \put(0,202.5){\makebox(0,0)[l]{\shortstack{\smallsc application\\[2mm]
\smallsc level}}}
  \thinlines
  \multiput(12.5,194.5)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(50,182.5){\makebox(80,15){\hvitalic planner internal representation
(IR)}}
  \thinlines
  \multiput(12.5,185.5)(10,0){14}{\line(1,0){5}}
  \thicklines
  \thinlines
  \multiput(12.5,172)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(35,175){\framebox(30,7.5){\parbox{15mm}{\smallsf\begin{center}IR
$\rightarrow$ SAR\end{center}}}}
  \put(115,175){\framebox(30,7.5){\parbox{15mm}{\smallsf\begin{center}SAR
$\rightarrow$ IR\end{center}}}}
  \thinlines
  \multiput(12.5,163)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(0,178.75){\makebox(0,0)[l]{\shortstack{\smallsc translation}}}
  \put(50,174){\vector(0,-1){13}}
  \put(130,161){\vector(0,1){13}}
  \put(50,160){\makebox(80,15){\hvitalic speech act representation
({\tiny${\cal N\!LL\/}$})}}
  \put(35,145){\framebox(30,15){\parbox{14mm}{\smallsf\begin{center}SPEECH
ACT\\ GENERATION\end{center}}}}
  \put(115,145){\framebox(30,15){\parbox{14mm}{\smallsf\begin{center}SPEECH
ACT\\ RECOGNITION\end{center}}}}
  \put(77.5,147.5){\line(0,1){10}}
  \put(102.5,147.5){\line(0,1){10}}
  \put(90,157.5){\oval(25,5)}
  \put(90,147.5){\oval(25,5)[b]}

%% FOLLOWING LINE CANNOT BE BROKEN BEFORE 80 CHAR
\put(90,150){\makebox(0,0){\parbox{11mm}{\smallsf\begin{center}MEMORY\end{center}}}}
  \put(66,152.5){\vector(1,0){10.5}}
  \put(76.5,152.5){\vector(-1,0){10.5}}
  \put(103.5,152.5){\vector(1,0){10.5}}
  \put(114,152.5){\vector(-1,0){10.5}}
  \put(150,145){\vector(-2,3){4}}
  \put(150,145){\line(0,-1){5}}
  \put(150,137.5){\makebox(0,0){\hvitalic SAR}}
  \put(150,135){\line(0,-1){55}}
  \put(150,80){\line(-2,-3){4}}
  \put(0,152.5){\makebox(0,0)[l]{\shortstack{\smallsc discourse\\[2mm] \smallsc
management}}}
  \thinlines
  \multiput(12.5,142)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(50,130){\makebox(80,15){\hvitalic semantic representation ({\tiny${\cal
N\!LL\/}$})}}
  \thinlines
  \multiput(12.5,133)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(50,144){\vector(0,-1){13}}
  \put(130,131){\vector(0,1){13}}

%% FOLLOWING LINE CANNOT BE BROKEN BEFORE 80 CHAR
\put(35,115){\framebox(30,15){\parbox{30mm}{\smallsf\begin{center}GENERATOR\\(SNL)\end{center}}}}
  \put(50,114){\vector(0,-1){3}}
  \put(35,95){\framebox(30,15){\smallsf FORMATTER}}

%% FOLLOWING LINE CANNOT BE BROKEN BEFORE 80 CHAR
\put(115,115){\framebox(30,15){\parbox{27mm}{\smallsf\begin{center}PARSER\\MORPHOLOGY\end{center}}}}
  \put(77.5,117.5){\line(0,1){10}}
  \put(102.5,117.5){\line(0,1){10}}
  \put(90,127.5){\oval(25,5)}
  \put(90,117.5){\oval(25,5)[b]}
  \put(90,120){\makebox(0,0){\smallsf GRAMMAR}}
  \put(103.5,122.5){\vector(1,0){10.5}}
  \put(68.5,122.5){\vector(-1,0){2.5}}
  \multiput(69.5,122.5)(2,0){4}{\line(1,0){1}}
  \put(130,112){\vector(0,1){3}}
  \put(115,95){\framebox(30,15){\smallsf SCANNER}}
  \put(50,94){\line(0,-1){4}}
  \put(50,80){\makebox(0,15){\hvitalic SNL}}
  \put(50,85){\vector(0,-1){4}}
  \put(130,90){\vector(0,1){4}}
  \put(130,80){\makebox(0,15){\hvitalic NL}}
  \put(130,81){\line(0,1){4}}
  \put(0,112.5){\makebox(0,0)[l]{\shortstack{\smallsc linguistic\\[1mm]
\smallsc core\\[2mm] \smallsc machinery}}}
  \thinlines
  \multiput(12.5,92)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(50,80){\makebox(80,15){\hvitalic (standardized) natural language}}
  \thinlines
  \multiput(12.5,83)(10,0){14}{\line(1,0){5}}
  \thicklines
  \put(35,65){\framebox(110,15){\hvdemi E-MAIL WRAPPER AND SCANNER}}
  \put(30,145){\line(2,3){4}}
  \put(30,80){\line(0,1){5}}
  \put(30,87.5){\makebox(0,0){\hvitalic SAR}}
  \put(30,90){\line(0,1){55}}
  \put(30,80){\vector(2,-3){4}}
  \thinlines
  \put(50,64){\vector(0,-1){18}}
  \put(95,46){\vector(0,1){18}}
  \put(130,46){\vector(0,1){18}}
  \put(0,72.5){\makebox(0,0)[l]{\shortstack{\smallsc e-mail\\[1mm] \smallsc
interface}}}
  \put(35,5){\framebox(30,40){}}
  \put(36,42.8){\begin{tiny}\parbox[t]{14mm}{\tinytt
    \setlength{\baselineskip}{0.8pt}
    \mbox{From:\ nerbonne@dfki.uni-sb.de}\\
    \mbox{To:\ hansu@coli.uni-sb.de}\\
    \mbox{Subject:\ COSMA:\ meeting request}\\[0.6mm]
    \mbox{Sehr geehrter Herr Uszkoreit,}\\[0.4mm]
    \mbox{Herr Nerbonne moechte mit Ihnen den}\\
    \mbox{folgenden Termin vereinbaren:}\\[0.3mm]
    \mbox{- Thema:\ `COSMA --- the future today'}\\
    \mbox{- Teilnehmer:\ John Nerbonne, ...}\\
    \mbox{- Art:\ Besprechung}\\
    \mbox{- Zeit:\ 19-May-1992, 11:00 h}\\
    \mbox{- Dauer:\ 1 bis 2 Stunden}\\
    \mbox{- Ort:\ DFKI}\\[0.3mm]
    \mbox{Koennen Sie diesen Termin wahrnehmen?}}\end{tiny}}
  \put(36,6.5){\begin{tiny}\parbox[b]{14mm}{\tinytt
    \setlength{\baselineskip}{0.8pt}
    \mbox{<cosma:\ begin sar>}\\
    \mbox{request(agent:\ nerbonne,}\\
    \mbox{\ \ \ \ \ \ \ \ hearer:\ hansu,}\\
    \mbox{\ \ \ \ \ \ \ \ action:\ arrange(agent:\ hansu,}\\
    \mbox{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ time:\ (?t | ),}\\
    \mbox{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ ...))}\\
    \mbox{<cosma:\ end sar>}}\end{tiny}}
  \put(80,23){\framebox(30,22){}}
  \put(81,42.8){\begin{tiny}\parbox[t]{14mm}{\tinytt
    \setlength{\baselineskip}{0.8pt}
    \mbox{Date:\ Mon, 18 May 92 10:32:38 +0200}\\
    \mbox{From:\ hansu@coli.uni-sb.de}\\
    \mbox{To:\ nerbonne@dfki.uni-sb.de}\\
    \mbox{CC:\ hinkelman@dfki.uni-sb.de}\\
    \mbox{Subject:\ Re:\ COSMA:\ meeting request}\\
    \mbox{In-Reply-To:\ <4712@dfki.uni-sb.de>}\\[0.6mm]
    \mbox{John,}\\[0.4mm]
    \mbox{ich bin einverstanden; ich werde}\\
    \mbox{versuchen puenktlich zu sein.}\\[0.4mm]
    \mbox{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ |:-)\ \ -\ \ hu}}\end{tiny}}
  \put(115,5){\framebox(30,40){}}
  \put(116,42.8){\begin{tiny}\parbox[t]{14mm}{\tinytt
    \setlength{\baselineskip}{0.8pt}
    \mbox{From:\ hinkelman@dfki.uni-sb.de}\\
    \mbox{To:\ nerbonne@dfki.uni-sb.de}\\
    \mbox{CC:\ hansu@coli.uni-sb.de}\\
    \mbox{Subject:\ Re:\ COSMA:\ meeting request}\\
    \mbox{In-Reply-To:\ <4712@dfki.uni-sb.de>}\\[0.6mm]
    \mbox{Sehr geehrter Herr Nerbonne,}\\[0.4mm]
    \mbox{Herr Uszkoreit ist mit dem von Ihnen}\\
    \mbox{vorgeschlagenen Termin}\\[0.3mm]
    \mbox{- Thema:\ `COSMA --- the future today'}\\
    \mbox{- Teilnehmer:\ John Nerbonne, ...}\\
    \mbox{- Art:\ Besprechung}\\
    \mbox{- Zeit:\ 19-May-1992, 11:00 h}\\
    \mbox{- Dauer:\ 1 bis 2 Stunden}\\
    \mbox{- Ort:\ DFKI}\\[0.3mm]
    \mbox{einverstanden.}}\end{tiny}}
  \put(116,6.5){\begin{tiny}\parbox[b]{14mm}{\tinytt
    \setlength{\baselineskip}{0.8pt}
    \mbox{<cosma:\ begin sar>}\\
    \mbox{inform(agent:\ hansu,}\\
    \mbox{\ \ \ \ \ \ \ hearer:\ nerbonne,}\\
    \mbox{\ \ \ \ \ \ \ action:\ accept(agent:\ hansu,}\\
    \mbox{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ ...))}\\
    \mbox{<cosma:\ end sar>}}\end{tiny}}
\end{picture}

